The Triple-Pair Construction for Weighted $\omega$-Pushdown Automata

Let S be a complete star-omega semiring and Sigma be an alphabet. For a weighted omega-pushdown automaton P with stateset 1...n, n greater or equal to 1, we show that there exists a mixed algebraic system over a complete semiring-semimodule pair ((S<<Sigma*>>)^nxn, (S<<Sigma^omega>>)^n) such that the behavior ||P|| of P is a component of a solution of this system. In case the basic semiring is the Boolean semiring or the semiring of natural numbers (augmented with infinity), we show that there exists a mixed context-free grammar that generates ||P||. The construction of the mixed context-free grammar from P is a generalization of the well known triple construction and is called now triple-pair construction for omega-pushdown automata.

==> eptcsdata.tex <==
\providecommand{\firstpage}{101}
\providecommand{\publicationstatus}{E. Csuhaj-Varj\'u, P. D\"om\"osi, Gy. Vaszil (Eds.): 15th International \\ Conference on Automata and Formal Languages (AFL 2017)\\
EPTCS 252, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.252.12}{10.4204/EPTCS.252.12}}

